Nonclassical Structures within the N-qubit Pauli Group

Structures that demonstrate nonclassicality are of foundational interest in quantum mechanics, and can also be seen as resources for numerous applications in quantum information processing - particularly in the Hilbert space of $N$ qubits. The theory of entanglement, quantum contextuality, and quantum nonlocality within the $N$-qubit Pauli group is further developed in this thesis. The Strong Kochen-Specker theorem and the structures that prove it are introduced and explored in detail. The pattern of connections between structures that show entanglement, contextuality, and nonlocality is explained. Computational search algorithms and related tools were developed and used to perform complete searches for minimal nonclassical structures within the $N$-qubit Pauli group up to values of $N$ limited by our computational resources. Our results are surveyed and prescriptions are given for using the elementary nonclassical structures we have found to construct more complex types of such structures. Families of nonclassical structures are presented for all values of $N$, including the most compact family of projector-based parity proofs of the Kochen-Specker theorem yet discovered in all dimensions of the form $2^N$, where $N\geq2$. The applications of our results and their connection with other work is also discussed.

==> abstract.tex <==



Structures that demonstrate nonclassicality are of foundational interest in quantum mechanics, and can also be seen as resources for numerous applications in quantum information processing - particularly in the Hilbert space of $N$ qubits.  The theory of entanglement, quantum contextuality, and quantum nonlocality within the $N$-qubit Pauli group is further developed.  The Strong Kochen-Specker theorem and the structures that prove it are introduced.  The pattern of connections between structures that show entanglement, contextuality, and nonlocality is explained.  Computational search algorithms and related tools were developed and used to perform complete searches for minimal nonclassical structures within the $N$-qubit Pauli group up to computation-limited values of $N$.  The complete results are presented, along with prescriptions for the enormous variety of ways that elementary nonclassical structures can be used to construct other types of nonclassical structures.  Families of nonclassical structures are presented for all values of $N$, including the most compact family of proofs the Kochen-Specker theorem yet discovered.  Many potential applications and connections to other work are also explored in detail 

==> preface.tex <==

\section*{Preface}

This thesis explores the issue of minimal nonclassical structures within the $N$-qubit Pauli Group and was prepared as a doctoral dissertation by Mordecai Waegell.  This research was supervised by P.K. Aravind at Worcester Polytechnic Institute.\newline

\begin{center}
	\textbf{Acknowledgements}
\end{center}

I thank first and foremost my adviser and friend P.K. Aravind, who first sparked my interest in the work of Bell and others on nonclassical physics, and who has provided me with insightful and supportive guidance throughout my tenure as his pupil.  Since my youth I have been inspired and fascinated by the illusions, patterns, and impossible figures conceived by M.C. Escher, so how fitting to find myself learning the physics of the impossible from a man with Escher prints and geometric baubles adorning his office.

I also thank the other readers of my thesis, Walter Lawrence and David Cyganski, with whom I have had interesting and enlightening conversations about the mysteries of quantum mechanics, and L. Ramdas Ram-Mohan who has graciously agreed to be part of my defense committee in lieu of Dr. Lawrence.

Next I thank Mladen Pavi\v{c}i\'{c} and Norman Megill for their insights and collaboration at various stages of this research.

Though we have never communicated directly, I would also like to acknowledge Asher Peres, David Mermin, Ad\'{a}n Cabello, and many others, whose work laid the foundations for what we have presented here.

Thanks to Sia Najafi of the WPI IT Department for giving us reliable access to good stable computers, on which we ran literally years of search algorithms.

Finally I would like to thank the Physics Department of Worcester Polytechnic Institute for supporting this work.

\clearpage



